A Framework for Approximating Qubit Unitaries

We present an algorithm for efficiently approximating of qubit unitaries over gate sets derived from totally definite quaternion algebras. It achieves $\varepsilon$-approximations using circuits of length $O(\log(1/\varepsilon))$, which is asymptotically optimal. The algorithm achieves the same quality of approximation as previously-known algorithms for Clifford+T [arXiv:1212.6253], V-basis [arXiv:1303.1411] and Clifford+$\pi/12$ [arXiv:1409.3552], running on average in time polynomial in $O(\log(1/\varepsilon))$ (conditional on a number-theoretic conjecture). Ours is the first such algorithm that works for a wide range of gate sets and provides insight into what should constitute a "good" gate set for a fault-tolerant quantum computer.

==> sec-cyclotomic.tex <==
%auto-ignore
%!TEX root = quaf.tex

\subsection{Cyclotomic fields}
We recall here some basic facts about cyclotomic fields, possibly for an appendix. 




Let $n\neq 2$ mod 4 be a positive integer.  Then $\bQ(\zeta_n)$ is the ray class field of $\bQ$ with conductor $(n)\infty$ and its real subfield $\bQ(\zeta_n)^+ = \bQ(\zeta_n + \zeta_n^{-1})$ is the ray class field with conductor $(n)$.  The subgroup of roots of unity is
\[\mu_{\bQ(\zeta_n)} = \begin{cases}
\mu_{n} & \text{ if } n \text{ is even} \\ 
\mu_{2n} & \text{ if } n \text{ is odd,}
\end{cases}\] 
where $\mu_F$ is the group of roots of unity in a field (necessarily a subgroup of the unit group $\bZ_F^\times$), and where $\mu_m = \vev{\zeta_m}\simeq \bZ/m$.  The discriminant of $\bQ(\zeta_n)$ is (Washington, Proposition 2.7)
\[(-1)^{\phi(n)/2} \frac{n^{\phi(n)}}{\prod_{p\mid n}p^{\phi(n)/(p-1)}},\]
where  $\phi(n) = |(\bZ/n)^\times|$ is {Euler's phi function}.    
For prime powers, this simplifies to $\ep p^{p^{n-1}(pn - n - 1)}$ with $\ep = -1$ if $p^n = 4$ or if $p \equiv 3$ mod  $4$ otherwise $\ep = 1$ (Washington Proposition 2.1).

If $n$ is divisible by more than one prime, then (Washington Proposition 2.8) $1 - \zeta_n \in \bZ[\zeta_n]^\times$ and 
\[\prod_{j \in (\bZ/n)^\times}(1-\zeta_n^j) = 1,\]
whereas  $1 - \zeta_{p^m} \notin \bZ[\zeta_{p^m}]^\times$ in the prime power case.
I seem to recall this having to do with the fact that the $n$th cyclotomic polynomial $\Phi_n(x) \in \bZ[x]$, for which $\bQ(\z_n) \simeq \bQ[x]/(\Phi_n(x))$, satisfies $\Phi_{p^m}(1) = p$ and $\Phi_n(1) = 1$ for composite $n$.  I recall this fact coming up when trying to determine conditions on $F$ so that $\leg{-1,-1}{F}$ contains a $\pi/n$-rotation, which led to the discovery that $U_{\mathbf k + 1 + \sqrt{2}}$ is the T-gate.

The following general result is Theorem 4.12 in Washington: 

\begin{quote}{\it Let $K$ be a CM field with real subfield $F$, let $\mu_K$ be the roots of unity in $K$ and define the map $\varphi \colon \bZ_K^\times \to \mu_K$ via $\varphi(u) = u/\bar u$.  
Then $[\mu_K:\mu_K^2] = 2$ and $\varphi(\mu_K \bZ_F^\times) = \mu_K^2$, whereas there are 
two possibilities: either
 $\bZ_K^\times = \mu_K\bZ_F^\times$ and $\varphi(\bZ_K^\times) = \mu_K^2$, or 
$[\mu_K^\times : \mu_K\bZ_F^\times] = 2$ and $\varphi(\bZ_K^\times) = \mu_K$. 
In other words, $[\bZ_K^\times:\mu_K \bZ_F^\times] \cdot [\mu_K:\varphi(\bZ_K^\times)] = 2.$}
\end{quote}


Corollary 4.13 of Washington then shows that $\varphi(\bZ[\zeta_{p^m}]^\times) =\mu_{\bQ(\zeta_{p^m})}^2$ so that $\bZ[\zeta_{p^m}]^\times = \mu_{\bQ(\zeta_{p^m})}\bZ[\zeta_n + \zeta_n^{-1}]^\times$, but if $n \not \equiv 2$ mod 4 is divisible by at least two primes, then $\varphi(\bZ[\zeta_n]^\times) = \mu_{\bQ(\zeta_n)}$ so that $[\bZ[\zeta_n]^\times: \bZ[\zeta_n + \zeta_n^{-1}]^\times \mu_{\bQ(\zeta_n)}] = 2$.

Define the subgroup of
\emph{cyclotomic units} 
\[C_n = \vev{-1,\zeta_n,\zeta_n^j -1: j = 1,\dotsc,n-1} \cap \bZ[\zeta_n]^\times\]
and let $C_n^+ = C_n \cap \bZ[\zeta_n]^+$.   These have finite index in $\bZ[\zeta_n]^\times$.  For prime powers, this is shown by Lemma 8.1 of Washington, which shows that $C_{p^m} = \mu_{p^m} C_{p^m}^+$ and  $C_{p^m}^+ = \vev{\xi_a : (a,p)  = 1, 1 < a < p^m/2}$, where $\xi_a = \zeta_{p^m}^{(1-a)/2} \frac{1 - \zeta_{p^m}^a}{1 - \zeta_{p^m}}$ satisfies $\pm \xi_a = \pm\frac{\sin(\pi a/p^m)}{\sin(\pi/p^m)} = \pm [a]_q$ with $q = \zeta_{p^m}$ and $\xi_{-a} = -\xi_a$.  Furthermore (Washington 8.2), $[\bZ[\zeta_{p^m} + \zeta_{p_m}^{-1}]^\times : C_{p^m}^+ ] = h^+_{p^m}$, where $h^+_{p^m}$ is the class number of $\bQ(\zeta_{p^m})^+$, conjecturally satisfying $h^+_{p^m} = h^+_{p^{m+1}}$ for all but finitely many $p^m$.  In particular, that $h^+_{2^m} = 1$ for all $m$ is known as Weber's class number conjecture, which to date has been proven for $m \leq 8$, and also for $m=9$ assuming the GRH.

When $n\not\equiv 2$ mod 4 is divisible by at least two distinct primes, the quantum integers $\pm \zeta_{n}^{(1-a)/2} \frac{1 - \zeta_{n}^a}{1 - \zeta_{n}}$ with $a \in (\bZ/n)/\{\pm 1\}$ may only generate a proper subgroup $C''_n$ of the real cyclotomic integers $C_n^+$.  There is a simple formula for the index (Washington 8.8)
\[[\bZ[\zeta_n + \zeta_n^{-1}]^\times : C''_n] = h_n^+ \prod_{\chi} \prod_{p\mid n}(1 - \chi(p)),\]
where the first product is over nontrivial even Dirichlet characters $\chi$ mod $n$, but if the RHS is zero then the index is infinite.  A larger subgroup $C_n' \subset C_n^+$ of real cyclotomic units can be defined in this case by including quantum integers at non-primitive $n$th roots of unity, and there is a more complicated formula (Washington 8.3) showing that $[\bZ[\zeta_n + \zeta_n^{-1}]^\times : C'_n]$ is finite.



==> sec-intro.tex <==
%auto-ignore
%!TEX root = quaf.tex

\section{Introduction}

One factor in scaling up quantum computing is the ability to compile complex quantum algorithms into sequences of instructions that a physical quantum computer can then execute fault-tolerantly. This requirement for compilation creates a need for methods that allow one to find short sequences of instructions whithout requiring
%and at the same time of and that at the same time do not lead to 
prohibitively-long compilation times. 

A complication is that good schemes for fault-tolerant quantum computing are not a dime a dozen. Universality aside, the various constraints that must be met---geometric locality, existence of a threshold error rate, and existence of an efficient decoding algorithm---significantly narrow the choices of schemes that can be implemented fault-tolerantly, for instance via distillation or via topologically protected operations such as braiding of quasiparticles. Among the main contenders are currently the surface code family and variations thereof, schemes based on concatenating short block codes, as well as schemes based on topological error protection. The choice of the scheme heavily influences the universal gate set that the quantum computer architect will have to work with.

Ideally, a compiler should abstract practical methods for quantum circuit synthesis and be able to support a wide variety of gate sets. Compilation should also account for tradeoffs between the total circuit size or depth, the number of required qubits, and the probability of leading to the correct result. As a long-term goal, a compiler should not only allow the translation of quantum programs into a variety of different elementary gate sets, but it should also inform the fault-tolerance layer of a quantum computer architecture about which choices of logical level gate sets would be preferable.

To the best of our knowledge, all known universal gate sets are number theoretic in nature, in the sense that the coefficients of the unitary transformations that make up the universal gates are all algebraic numbers. Examples include (i) the Clifford+$T$ basis that  arises e.g. from the surface code \cite{Fowl12f} and the concatenated Steane \cite{Stea96,Stea03b} code, 
%where in both cases the field is the cyclotomic field $\q(\omega_8)$. The generating set in this case can be chosen to be the single-qubit Hadamard ($H$) and $T$ gates, given by $ H = \frac{1}{\sqrt{2}} \, \left[\begin{smallmatrix}1&1\\1&\textrm{-}1\end{smallmatrix}\right]$,and $T_8 = \left[\begin{smallmatrix}1&0\\0&e^{i \pi/4}\end{smallmatrix}\right]$.
%Another example is the so-called 
(ii) the Clifford$+\pi/12$ basis that arises from e.g. from quantum computing with metaplectic anyons \cite{CW:2014,CBK+:2015}, 
%where the field is the cyclotomic field $\q(\omega_{12})$, 
(iii) the Fibonacci basis that 
%which is defined over $\q(\omega_{10})$ and which 
arises from Fibonacci anyons \cite{FLW:2002,NSF+:2008}, and 
(iv) the gate set that consists of Clifford gates augmented by (distilled) Fourier angles,
%$T_{2^n} = \left[\begin{smallmatrix}1&0\\0&e^{i \pi/2^{n-1}}\end{smallmatrix}\right]$. The latter gate set arise e.g. from offline state distillation protocols that create equatorial states of the form $\frac{1}{\sqrt{2}}(\ket{0}+e^{i \pi/2^{n-1}}\, \ket{1})$ which then can be used to implement $T_{2^n}$, 
see e.g., \cite{DP:2015}. 
%Here the field is the cyclotomic field $\q(\omega_{2^n})$, where $n\geq 2$.
In all these cases, the coefficients of the gates are algebraic integers and actually lie in a cyclotomic field $\q(\zeta_n)$ for some $n\in\n$ or its degree two extension. 

As a finite set of gates can at best generate an infinite, yet discrete subgroup of U(2), several questions arise rather naturally: is the group generated by unitaries from the gate set dense in $U(2)$ or not. When this is the case the gate set is called universal. The next question is how long the circuit over the gate set should be 


Recently, further classes of universal ``Golden Gates" were proposed by Sarnak \cite{Sarnak:2015}, who also analyzed the constants in the expansion properties of these gate sets. Understanding universal gate sets with algebraic entries is the goal of this paper, in particular as it relates to efficient algorithms for compilation. 


\mypar{Previous work} The Solovay-Kitaev algorithm \cite{KSV:2002,DN:2005} provides a solution to the approximate synthesis problem that is very general in that it is applicable to  any approximately universal gate set. For a given target approximation precision $\varepsilon$ and a given target unitary the algorithm from the reference implementation of the Solovay-Kitaev algorithm in \cite{DN:2005} outputs a circuit of size $O(\log^{3.97} (1/\varepsilon))$. The number of operations needed to compile said circuit is also polylogarithmic in $\varepsilon$ and can be bounded by $O(\log^{2.71}(1/\varepsilon))$.

A natural question is whether this is the best possible bound, both, for circuit size and compilation time. Using arguments from harmonic analysis and expanders it is possible to show the existence of significantly shorter factorizations for many gate sets, albeit non-constructively. The connection uses the observation that a spectral gap property of an operator $\Omega$ that can be defined for any given gate set ${\mathcal G}$ implies
efficient universality \cite{H1}. More precisely, the averaging operator $\Omega: f \mapsto \overline{f}$ is a Hermitian linear operator defined on functions from $L^2(SU(d))$ as
\[
\Omega(f) = x \mapsto \overline{f}(x) = \frac{1}{|{\mathcal G}|} \sum_{g \in {\mathcal G}} \left(f(gx) + f(g^\dagger x)\right).
\]
It is easy to see that $1$ is always an eigenvalue of $\Omega$ as each constant function is mapped to itself under $\Omega$ and this is the largest eigenvalue, i.e., $\lambda_1=1$. More interesting is the behavior of the eigenvalues that are less than $1$, in particular whether there is a gap between $\lambda_1$ and $\lambda_2$, where $\lambda_2$ is the second largest eigenvalue. It is said that $\Omega$ has a {\em spectral gap} \cite{S1,S2} if the supremum over the eigenvalues for all non-constant functions is strictly less than $1$. Cases of gate sets ${\mathcal G}$ for which the corresponding averaging operator $\Omega$ has a spectral gap are extremely useful as it is known that this automatically implies efficient approximation \cite{S1,S2,H1} in the following sense: consider the set ${\mathcal G}^n$ that consists of products of gates ${\mathcal G}$ of length $n$. It is known that if $\Omega$ has a spectral gap, then the operator $\Omega^n$, which is obtained by applying $\Omega$ to a given function $f$ a number of $n$ times, converges exponentially fas to average $\int f(x) d \mu(x)$ with respect to the Haar measure. Using this property, in \cite{H1} it was shown that this implies that if a gate set ${\mathcal G}$ has a spectral gap then this immediately implies that for any given target unitary $U$ and any given target $\epsilon > 0$ there exists a word $ w \in {\mathcal G}^n$ of length $n$ where $n=O(\log(1/\varepsilon))$ such that $\|w - U \| < \epsilon$.

It was shown in \cite{H1} that efficient universality follows from the spectral gap property of the averaging operator over a finite, dense set of unitaries ${\mathcal G}$. A natural question is whether having a spectral gap is a rare or a rather common property for a given gate set that generates a dense subgroup of $SU(d)$ to have. Perhaps, surprisingly, it turns out that as long as the all matrix elements of all elements of ${\mathcal G}$ are {\em algebraic numbers}, i.e., they all lie within an algebraic extension $K$ of the rational numbers $\q$,
automatically the gate set has a spectral gap \cite{B1,B2}. Up to basis change, this set of universal gates with algebraic entries comprises the only class of universal gate sets that is known to us as arising from fault-tolerant quantum error correction protocols, respectively from braiding, fusion, and measurement protocols for non-abelian quasiparticles. What is particularly tantalizing about Bourgain and Gamburd's result is that it is not obvious at all how to efficiently find the short factorizations that are known from the spectral gap property to exist. The purpose of this paper is to show that at least for some gate sets that give rise to positive definite quaternion algebras over so-called CM fields of bounded class number, then an efficient algorithm for quantum compilation can be derived.

Previous successes in compiling are mainly restricted to specific gate sets. This includes the works on synthesis for the Clifford$+T$ gate set by Selinger \cite{S}, Kliuchnikov/Maslov/Mosca \cite{KMM2,KMM3}, and Ross/Selinger \cite{RS}. Historically, the Clifford$+T$ gate set was the first gate set for which it was shown that it is possible to find efficient factorizations in polynomial time. It should be noted that these algorithms are efficient modulo some number-theoretic conjectures which however in practice do not seem to impact the run-time of the algorithm, even for very small $\epsilon$ of the order $10^{-18}$ or smaller.
See also \cite{Kliuchnikov:2014} for an overview. Also for the case of the Clifford$+V$ basis \cite{BGS}, and for Fourier angles \cite{SGKM}, as well as for so-called RUS circuits \cite{BRS:2015,BRS:2015b} similar results are known.

%In the case of the Clifford$+T$ gate set---and similarly for the other mentioned gate sets, albeit with different constants and different additive terms---the resulting circuits has scaling close to the information-theoretic lower bound of $3\log_2(1/\varepsilon)$
% for $z$-rotations, see \cite[Section 9]{S}. For general rotations, Euler decompositions can be used to obtain an upper bound of $9 \log_2(1/\varepsilon)$ which is the best known circuit size for unitary decompositions.

\mypar{Our contribution} Our main innovation is a framework for ancilla-free, approximate synthesis of unitary transformation that is applicable to many gate sets. The general approach is shown in Figure \ref{fig:algoOverview}. Features of our approach are that a) it is applicable to a wide range of gate sets, including several infinite families of gates, b) it provides a natural and unified explanation for all the synthesis algorithms that have been found as point-solutions for the previously mentioned gate, c) the algorithms that comprise our framework are all efficient, under some natural assumptions about the underlying gate set, and finally d) our method has been implemented in the computer algebra system Magma \cite{MAGMA:1997}, thereby giving a proof of principle that the proposed algorithms actually work reasonably fast in practice.

An important distinction that is germane to our framework is that there are computations that can be performed offline, i.e., those are computations that depend on the underlying gate set alone and not on the input target rotation, the accuracy etc. Those inputs will then be handled during an online phase in which the bit-size of the input matters, the target precision matters, etc. Furthermore, it is important to note that the synthesis part of the algorithm proceeds in a two-step fashion, similarly to earlier approaches \cite{S,KMM2,KMM3,RS} however with a much broader target of applicability: in a first stage, an approximation to the given unitary is computed in such a way that the approximating unitary can be considered to be an element of quaternion algebra over $F$. In a secondary step, then said quaternion is decomposed using an exact synthesis method.

We will describe all stages of the algorithms described in Figure \ref{fig:algoOverview} in great detail in the following sections of the paper, however, the following might be a guiding intuition about what the phases entail. The offline computation in part a) of the figure includes the computation of such quantities (here denoted in summary as ``infrastructure ${\mathcal A}$'') as the number field $K$ over which the gates in ${\mathcal G}$ are defined, the real and complex embeddings of $K$, the totally real subfield $F$ of $K$, the ring of integers $\z_K$, the conductor of $K$, and the unit group of $\z_K$, and a quaternion algebra $Q$ defined over $F$. It should be noted that we treat $K$ as being a constant, i.e., all offline computations are assumed to have constant cost. This allows us to stay clear of hard computational problems in algebraic number theory which all become easy for {\em constant} extensions.

\begin{figure}[hbt]
{
  \centering
  \makeatletter
\pgfdeclareshape{datastore}{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north west}
  \backgroundpath{
    %  store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
 }
}
\tikzset{align at top/.style={baseline=(current bounding box.north)}}

\makeatother
\usetikzlibrary{arrows}

\begin{tabular}{cc}
\raisebox{1.98cm}{
\begin{tikzpicture}[
  every matrix/.style={ampersand replacement=\&,column sep=0cm,row sep=0.25cm},
  heading/.style={draw,very thick,shape=rectangle,fill=gray!10,inner sep=.3cm},
  sink/.style={draw,thick,rounded corners,fill=gray!20,inner sep=.2cm},
  datastore/.style={draw,very thick,shape=datastore,inner sep=.1cm},
  to/.style={->,>=stealth',shorten >=1pt,semithick},
  every node/.style={align=center}]
  % Position the nodes using a matrix layout
\tikzset{align at top/.style={baseline=(current bounding box.north)}}
  \matrix{
	\node[heading] (head) {{\bf Offline component}}; \\[1ex]
    \node[datastore] (input) {Input: Universal gate set ${\mathcal G}$}; \\
    \node[sink] (pre) {Precomputation}; \\
    \node[datastore] (infra) {Output: Infrastructure ${\mathcal A}$}; \\
};
%	\draw[to] (head) --(input);
	\draw[to] (input) --(pre);
	\draw[to] (pre) --(infra);
\end{tikzpicture}
}&
\begin{tikzpicture}[
  every matrix/.style={ampersand replacement=\&,column sep=0cm,row sep=0.25cm},
  heading/.style={draw,very thick,shape=rectangle,fill=gray!10,inner sep=.3cm},
  sink/.style={draw,thick,rounded corners,fill=gray!20,inner sep=.2cm},
  datastore/.style={draw,very thick,shape=datastore,inner sep=.1cm},
  to/.style={->,>=stealth',shorten >=1pt,semithick},
  every node/.style={align=center}]
  % Position the nodes using a matrix layout
  \matrix{
	\node[heading] (head) {{\bf Online component}}; \\[1ex]
    \node[datastore] (input) {Input: Target $U$, precision $\varepsilon$, infrastructure ${\mathcal A}$};\\
    \node[sink] (approx) {Approximation algorithm};\\
    \node[datastore] (exact) {Quaternion $q$ over algebraic number field $F$};\\
    \node[sink] (synth) {Exact synthesis algorithm};\\
    \node[datastore] (circuit) {Output: Circuit approximating $U$ over ${\mathcal G}$ within $\varepsilon$};\\
};
%	\draw[to] (head) --(input);
	\draw[to] (input) --(approx);
	\draw[to] (approx) --(exact);
	\draw[to] (exact) --(synth);
	\draw[to] (synth) --(circuit);
\end{tikzpicture} \\
a) & b)
\end{tabular}
\caption[Compilation algorithm]{High level overview of the algorithms used in this paper to solve the unitary approximation problem (UAP): a) Precomputation of infrastructure data ${\mathcal A}$ related to the given universal gate set ${\mathcal G}$ in an offline component, (b) Synthesis of a circuit over the given gate set as an online component: synthesis is performed as a two step process in which first an element $q$ of a quaternion algebra defined over an algebraic number field $F$ is produced which in a precise mathematical sense can be considered an approximation to the given unitary $U$. Then in a subsequent step an exact synthesis method is used to find the factorization into a quantum circuit.}
\label{fig:algoOverview}
}
\end{figure}

Next, the approximation part of the online computation in part b) of the figure involves a rescaling of the set of possible approximating unitaries in such a way that we can chose them from a convex polytope that is ``balanced'' in a suitable sense. In order to achieve approximate balancedness, we have to rescale the coefficients of unitaries by units in $\z_K$, where the choice of a good rescaling leads to a closest vector problem in a lattice generated by the logarithms of the fundamental units of $\z_K$. To solve this problem approximately, we compute reduced bases for the lattice, such as the ones produced by the LLL algorithm and its recent improvements. Finding a feasibly approximating unitary however also entails a purely number-theoretic step in which we seek to find a suitable quaternion that approximates the target unitary. For this step a so-called {\em relative norm equation} must be solved for some elements in $F$, i.e., we must find algebraic integers in $\z_K$ that hit those target numbers under the norm map. Generally, solving norm equations is difficult and even in our case where the extension $K$ is assumed to be constant, it is a non-trivial task to solve the relative norm equations. Our approach is to focus on instances that arise with high probability\footnote{Assuming a number-theoretic conjecture. See Section \ref{sec:conjecture} for discussion and Section \ref{sec:examples} for experimental evidence.} and that turn out to be treatable by an efficient algorithm.

Once an approximating unitary corresponding to an element of a maximal order in a quaternion algebra has been found, a secondary synthesis stage kicks in where an exact synthesis algorithm factors the quaternion into a product of elementary quaternions which correspond to elementary gates. This piece of the algorithm has been described in \cite{KY1} but we provide a short summary of this method to make our paper self-contained apart from the technical details given in \cite{KY1}.

It is instructive to compare the Solovay-Kitaev algorithm \cite{KSV:2002,DN:2005} with our framework shown in Figure \ref{fig:algoOverview} as at the high-level there are some similarities but also striking differences: a common feature between both approaches is that they naturally decompose into an offline and an online phase: in case of Solovay-Kitaev, the offline phase consists in producing an initial net which typically is obtained by taking the entirety of all words up to a certain length. This leads to large memory overheads but is completely independent of the problem instance that we later want to solve, i.e., the target rotation and the approximation parameter $\varepsilon$. The online phase in Solovay-Kitaev consists in looking up the target gate within a database of already produced circuits and, in case this lookup fails, a refinement phase of the net.

All known implementations of the Solovay-Kitaev algorithm suffer from the enormous memory footprint which comes with the computation of the database of approximating words and from the plateau-like behavior in terms of approximation quality, i.e., there is no graceful degradation of run-time with the target precision but rather long plateaus with no improvement, followed by large jumps that are computationally and memory intensive. On the other hand, the number theoretic approach developed in our paper has an offline phase that is entirely number theoretical, and for all practical gate sets that have been proposed so far as universal fault-tolerant gates, can be done easily. Our online phase has essentially no memory footprint at all. For the rounding  we use approximate solution to a Closest Vector Problem in the log-unit lattice for a number field, followed by the solution of a relative norm equation. By using the fact that the degree of the arising number fields are constant we show that all these computations can be done in probabilistic polynomial on a classical computer. 

The main benefit of our method when compared to approaches based on $\varepsilon$-nets and the Solovay-Kitaev theorem is that the factorizations found are of length $O(\log(1/\varepsilon))$, where moreover the constant in front of the $\log(1/\varepsilon)$ term can be characterized by intrinsic properties of the underlying gate set. The main benefit of Solovay-Kitaev still is its broad applicability, i.e., if a gate set does not meet the requirements that we impose of essentially corresponding to a maximal order in a quaternion algebra, then to the best of our knowledge there is no better approach known than the Solovay-Kitaev theorem.

\subsection{Ancillae free approximation} Formally the problem of ancillae free approximation for single qubit gate sets can be stated as follows:

% TODO:  State Closest unitary problem , discuss Ross-Selinger, brute force and \cite{KMM3}. Discuss its relaxation.

% TODO: Now we explain how to obtain the cost bound function for brute force search algorithms. $\td$

\begin{prob}[unitary approximation problem in two dimensions, UAP]\label{prob:uap}
Given
\begin{enumerate}
\item finite universal unitary gate set $G \subset U(2)$
\item cost function $c:G\rightarrow \r^{+}$ ($c:G\rightarrow\set{1}$ corresponds to circuit length)
\item distance function $\rho$ on the set of unitaries
\item cost bound function $C_{\max}: \r^{+} \rightarrow \r^{+}$
\item target unitary $U$ from $U_{targ} \subset U(2)$
\item target precision $\ve$
\end{enumerate}
Find $\rg{g_1}{g_N}$ from $G$ such that $\rho\at{\trg{g_1}{g_N},U} \le \ve$ and $\sum_{k=1}^{N} c\at{g_k} \le C_{\max} \at{\ve} $.
\end{prob}
We say that the algorithm solves UAP in polynomial time, if it solves Problem \ref{prob:uap} for arbitrary unitaries $U$ from $U_{targ}$ and its runtime is polynomial in $\log(1/\ve)$. We also allow to spend arbitrary time on precomputation based on (1) -- (4) and store arbitrary amount of results of the precomputation. The set $U_{targ}$ can be equal to $U(2)$ or some its subset. For example, it can be the set of all unitaries $e^{i \vp Z}$ for $Z$ being Pauli $Z$ matrix and $\vp$ being arbitrary real number.

The hardness of solving UAP and the existence of the solution to it depends on the choice of cost bound function $C_{\max}$. We summarize known algorithms for solving UAP in Table~\ref{tab:algo}. In practice, for target precisions $10^{-10}$ to $10^{-30}$, the overhead from using the Solovay Kitaev algorithm can be between one to three orders of magnitude. On the other hand, the methods based on brute force search find the best possible solution, but are frequently limited to precisions $10^{-5}$ or even less because their runtime and required memory scale exponentially with $\log(1/\ve)$. Methods \cite{RS,S,BGS} together with the one that is the focus of this paper (see also Table~\ref{tab:algo}, lines 3-8) are based on exact synthesis algorithm and produce results that has cost bound similar to brute force search but have polynomial runtime. In the next subsection we will explain the idea of this methods in more detail.

\begin{table}
{\small
\begin{centering}
\input{table-uap-algorithms.pgf}
\end{centering}
\caption{\label{tab:algo} Known algorithms for solving the unitary approximation problem (UAP).}
}
\end{table}

% Discuss the best possible solutions to UAP

\subsection{Approximation methods based on exact synthesis} \label{sec:esmethods}

Algorithms that solve UAP~(Problem~\ref{prob:uap}) and that are based on the exact synthesis algorithm (see Table~\ref{tab:algo}, lines 3-8) can be described by the flow chart on Figure~\ref{fig:online-flow}. The focus of this paper is such an algorithm that works for gate sets described by an arbitrary {\em totally definite} quaternion algebra and generalizes algorithms from \cite{S,BGS} (see also Table~\ref{tab:algo}, lines 3-6). We leave the analog of the algorithm for indefinite quaternion algebras for future work. In this subsection we first discuss what does it mean for the gate set to be described by totally definite quaternion algebra and next look at the flow on Figure~\ref{fig:online-flow} in more details.

We refer to Section~\ref{sec:basics} for definitions and more details discussion of mathematical objects discussed below. The aim of this part to explain connections between them and to the algorithm presented in this paper on a high level. We say that the gate set $G$ is described by quaternion algebra if the following list of objects can be specified and related to the gate set.

\begin{restatable}{dfn}{qgc}
\label{dfn:quaternion-spec} A quaternion gate set specification is a tuple $\ip{F,\s,a,b,\mo,S}$ where:
\begin{itemize}
\item $F$ is a totally real number field and  $\s$ is an embedding of $F$ into $\r$
\item $a,b$ are elements of $F$ that define the quaternion algebra $\at{\frac{a,b}{F}}$ over $F$
\item $\mo$ is a maximal order of $\at{\frac{a,b}{F}}$ 
\item $S=\set{\p_1,\ldots,\p_M}$ is a set of prime ideals of $F$
\end{itemize}
\end{restatable}
Using the embedding $\s$ any quaternion $q$ from the quaternion algebra can be mapped to a special unitary $U_q \in SU(2)$. We discuss the precise construction of this map in Subsection~\ref{sec:quat-and-unitaries}. This map has the following important properties:
\[
 U_{q_1 q_2 } = U_{q_1} U_{q_2} , U^{\dagger}_{q}=U_{q^\ast}
\]
where $q^{\ast}$ is the conjugate of $q$. Let us also define the following closed under multiplication set
\[
\mo_S = \set{ q \in \mo : \nrd\at{q}\z_F = \trg{\p_1^{L_1}}{\p_M^{L_M}}, L_k \in \z,\,L_k \ge 0  },
\]
and call $\at{L_1,\ldots,L_M}$ the {\em cost vector} of $q$. Above $\nrd\at{q}$ is the reduced norm of quaternion and $\z_F$ is a ring of integers of number field $F$. The set $\mo_S$ is closed under multiplication because $\mo$ is closed under multiplication and $\nrd\at{q_1 q_2} = \nrd\at{q_1} \cdot \nrd\at{q_2}$.

A simplified set of conditions that must hold for the gate set to be described by the quaternion gate set specification is:
\begin{enumerate}
\item There must exist subset $G_Q$ of $\mo_S$ such that $G=\set{U_q : q \in G_Q }$.
\item The group generated by $G$ must be equal to group $\set{U_q : q \in \mo_S }$.
\end{enumerate}
Condition (1) implies that group generated by elements from $G$ is a subgroup of $\set{U_q : q \in \mo_S }$. Condition (2) can be checked using the framework developed in the recent paper~\cite{KY1} given set $G_Q$. We will give a brief overview of results in~\cite{KY1} in Subsection~\ref{sec:qfes-review}. One way of checking the condition is to first compute a finite set of quaternions $G_Q^{\star}$ such that every element of $\mo_S$ can be written as a product of elements of $G_Q^{\star}$  and a scalar (using algorithms from~\cite{KY1}). We will say that $G_Q^{\star}$ generates $\mo_S$. Second, for each $q$ from $G_Q^{\star}$ find a representation of $U_q$ as a product of elements of $G$. For all $q$ from $G_Q^{\star}$ we then can define:
\begin{equation}
\crt\at{q} = (U_1, \ldots, U_n) , \text{ where } U_q = U_1 \ldots U_n , U_k \in G. \label{eq:circuit}
\end{equation}
One way of defining the cost of elements of $G_Q^{\star}$ is
\[
c\at{q} = \sum_{k=1}^n c\at{U_k}.
\]
To summarize we give the following definition:
\begin{restatable}{dfn}{qag}
\label{dfn:qag} We say that a gate set $G$ is described by quaternion algebra if the following data is defined:
\begin{enumerate}
\item A quaternion gate set specification $\ip{F,\s,a,b,\mo,S}$,
\item A set of quaternions $G_Q^{\star}$ that generates $\mo_S$,
\item A map $\crt$ as described by equation (\ref{eq:circuit}).
\end{enumerate}
\end{restatable}

In Section~\ref{sec:examples} we will give examples of the gate sets described by quaternion algebras (including Clifford$+T$ and $V$ basis) and will explicitly specify (1)--(3) for each example. Now we have enough background to discuss the flow of our algorithm in more details.

Steps 2 and 3 in Figure~\ref{fig:online-flow} are the crucial in the algorithm. For simplicity we focus on the case when set $S$ consists of only one prime ideal. Our input to Step 2 is $L_1,\vp,\ve$. The output of Step 2 is a quaternion $q$ from $\mo_S$ such that its cost is equal $L_1$ and $U_q$ is within distance $\ve$ from $R_z\at{\vp}$. The fact that our target gate set $G$ is described by quaternion algebra (Definition~\ref{dfn:qag}) immediately implies that $U_q$ can be expressed as a circuit over $G$. Steps 3 and 4 construct such a circuit. In Step 3 we express $q$ as a product $q_1\ldots q_n$ of elements of $G_Q^{\star}$ and a scalar from $F$ using exact synthesis algorithm described in~\cite{KY1}. In Step 4 we find a circuit for $U_q$ over gate set $G$ as concatenation of circuits for each $q_k$.

Let us now discuss Step 1 in more detail. To give some intuition we start with the Clifford+T gate set example~(analyzed in more details in Section~\ref{sec:examples}). In this case set $S$ contains precisely one prime ideal $\p_1$ and $L_1$ is greater or equal to the T-count of the resulting circuit. To ensure that approximation step succeeds the input to the algorithm must satisfy inequality
\[
L_1\log\at{N\at{\p_1}} \ge 4\log(1/\ve) + C \text{, where } N\at{\p_1} \text{ is the norm of } \p_1.
\]
This reproduces result in~\cite{S} that the $T$-count scales as $4 \log_2(1/\varepsilon) + C$  because $N(\p_1)=2$ holds for the Clifford$+T$ case. The bound also saturates the lower bound proved in~\cite{S} up to an additive constant. In this simple case, in Step 1 of Figure~\ref{fig:online-flow} we just assign $L_1 = \ceil{ (4\log(1/\ve) + C)/\log\at{N\at{\p_1}} }$. In our algorithm we precompute constant $C$ based on quaternion gate set specification.

More generally, the cost vector $\at{L_1,\ldots,L_M}$ that we input to Step 2 must satisfy the following inequality
\[
L_1\log\at{N\at{\p_1}} + \ldots + L_M\log\at{N\at{\p_M}} \ge 4\log(1/\ve) + C.
\]
The length of the circuit output by our algorithm is proportional to $L_1 + \ldots + L_M$ and therefore proportional to $\log(1/\ve)$ which is up to multiplicative factor is the best possible. Cost optimality up to an additive constant is more subtle and is dependent on the choice of cost function and the gate set. We will discuss this more in Section~\ref{sec:examples}.


\begin{figure}[ht!]
\rule[0.5ex]{1\columnwidth}{1pt}

\begin{centering}
\input{chart-approximation-flow.pgf}
\par\end{centering}

\rule[0.5ex]{1\columnwidth}{1pt}

\caption{\label{fig:online-flow} High level flow of the approximation process. }
\end{figure}

In some cases we might not have very fine control of the cost of output circuit using cost vector. In the worst case cost vector will allows us to control the cost of the output circuit up to multiplicative factor. In this situation we can use the following strategy to improve the cost of output
\begin{itemize}
\item In Step 1 make a request for several cost vectors
\item In Step 2 for each cost vector request several quaternions that achieve required quality of approximation
\item In Step 4 try to optimize final circuits using rewriting rules for gate set $G$ and pick the ones with minimal cost. Rewriting rules for the gate set $G$ can be obtained using exact synthesis framework~\cite{KY1}.
\end{itemize}

% \subsection{Short overview of the paper}


